A Projected Gradient Method for Opinion Optimization with Limited Changes of Susceptibility to Persuasion

Many social phenomena are triggered by public opinion that is formed in the process of opinion exchange among individuals. To date, from the engineering point of view, a large body of work has been devoted to studying how to manipulate individual opinions so as to guide public opinion towards the desired state. Recently, Abebe et al. (KDD 2018) have initiated the study of the impact of interventions at the level of susceptibility rather than the interventions that directly modify individual opinions themselves. For the model, Chan et al. (The Web Conference 2019) designed a local search algorithm to find an optimal solution in polynomial time. However, it can be seen that the solution obtained by solving the above model might not be implemented in real-world scenarios. In fact, as we do not consider the amount of changes of the susceptibility, it would be too costly to change the susceptibility values for agents based on the solution. In this paper, we study an opinion optimization model that is able to limit the amount of changes of the susceptibility in various forms. First we introduce a novel opinion optimization model, where the initial susceptibility values are given as additional input and the feasible region is defined using the $\ell_p$-ball centered at the initial susceptibility vector. For the proposed model, we design a projected gradient method that is applicable to the case where there are millions of agents. Finally we conduct thorough experiments using a variety of real-world social networks and demonstrate that the proposed algorithm outperforms baseline methods.

==> src/analysis.tex <==
\section{Analysis}\label{sec:analysis}

% \begin{lemma}
%   Assume that $f$ has an $L$-Lipschitz continuous gradient.
%   Then, \Cref{alg:PGM} terminates after $O(L \epsilon^{-2})$ computation of $f$ and $\nabla f$,
%   and outputs a point $x \in \mathcal C$ such that $\norm{\mathcal G_\eta(x)} \leq \epsilon$ for some $\eta > 0$.
% \end{lemma}


==> src/observation.tex <==
\section{Basic Observations}\label{sec:observation}
In this section, we present basic observations that are useful for designing our projected gradient algorithm. 


\subsection{Gradient and Hessian Matrix of Objective Function}



\Ja{
$\odot$ は成分ごとの積．
下の補題は前の節の式からすぐ出ますね．
\begin{lemma}
  Let $M =I - \mathrm{Diag}(\1 - \bm{\alpha}) P$. Then it holds that 
  \begin{align}
    \nabla f(\bm{\alpha})
    = (M^{-\top} \bm 1) \odot \prn[\big]{\bm{s} - P M^{-1} (\bm{\alpha} \odot \bm{s}) },
    \label{eq:grad_f}
  \end{align}
\end{lemma}
（$M$ の定義が前節までと違っています）
\begin{proof}
  Let $P = [p_1,\dots,p_n]^\top$ and $\bm{v} = M^{-\top} \bm 1$. 
  As $f(\bm{\alpha}) = \bm{v}^\top (\bm{\alpha} \odot \bm{s})$ holds, we have 
  \begin{align}
    \frac{\partial f}{\partial \alpha_i}
    = \frac{\partial \bm{v}^\top}{\partial \alpha_i} (\bm{\alpha} \odot \bm{s}) 
    + v_i s_i. \label{eq:f_partial_alpha_i}
  \end{align}
  On the other hand, differentiating both sides of $\bm{v}^\top M  = \bm 1^\top$ with respect to $\alpha_i$, we have 
  \begin{align*}
    \bm{v}^\top \frac{\partial M}{\partial \alpha_i}
    + \frac{\partial \bm{v}^\top}{\partial \alpha_i} M
    = \0^\top, 
  \end{align*}
  which implies that 
  \begin{align}
    \frac{\partial \bm{v}^\top}{\partial \alpha_i}
    = - \bm{v}^\top \frac{\partial M}{\partial \alpha_i} M^{-1}
    = - v_i p_i^\top M^{-1}. 
    \label{eq:vt_partial_alpha_i}
  \end{align}
  Combining the equations \eqref{eq:vt_partial_alpha_i} and \eqref{eq:f_partial_alpha_i}, we have 
  \begin{align}
    \frac{\partial f}{\partial \alpha_i}
    = v_i \prn[\big]{
      s_i - p_i^\top M^{-1} (\alpha \odot s)
    }, 
  \end{align}
  which is equivalent to the equation~\eqref{eq:grad_f}. 
\end{proof}
これなら逆行列は必要なく，線形方程式を 2 回解くだけでよい．
}



\subsection{Lipschitz Continuity of Gradient}

Here we show the Lipschitz continuity of the gradient of the objective function $f$ over the feasible region $\mathcal{C}$.
To this end, we first prove that $\|\nabla^2 f(\bm{\alpha})\|_2$ is bounded.
The following lemma is useful:

\begin{lemma}[A part of Lemma 3.1 in Chan et al.~\cite{Chan+19}]\label{lm51}
%\begin{lemma}[Lemma 5.1 ~\cite{abebe2020ropinion}]\label{lm51}
Let $\bm{\alpha} \in (0, 1)^V$ and $K \subsetneq V$.
%$A=\mathrm{Diag}(\bm{\alpha})$ ($\bm{\alpha} \in (0, 1)^V$).
Then there exists a matrix $M_K$ such as
\begin{align*}
 M_K = (I -(I-A_{-K})P)^{-1},
\end{align*}
where $A_{-K}$ is the matrix constructed from $A$ by setting $A_{ii}=0$ for every $i \in K$.
Moreover, every element of $M_K$ is positive.
\end{lemma}


\begin{lemma}\label{lem:boundedness}
Let $\bm{\alpha} \in (0, 1)^V$.
If $\bm{\alpha}$ has at least one element whose lower bound is positive, then $\|\nabla^2 f(\bm{\alpha})\|_2$ is bounded.
\end{lemma}

\begin{proof}
  Let $\bm{z}$ such as $f(\bm{\alpha}) = \sum^{n}_{k=1} z(\bm{\alpha})$.
  From the calculation in Lemma 5.2~\cite{abebe2020ropinion}, the gradient of $\bm{z}(\bm{\alpha})$ and $M$ is represented by below.
  \begin{equation*}
    \begin{aligned}
      \frac{\partial z(\boldsymbol \alpha)}{\partial \alpha_i} &= M\bm{e}_{i}\bm{e}_{i}^\top( \bm{s} - P z(\bm{\alpha})) \\
      \frac{\partial M}{\partial \alpha_i} &= -M\bm{e}_i\bm{e}_{i}^\top PM
    \end{aligned}
  \end{equation*}

  Using these results, the Hessian of $z$ is represented by below.
  \begin{equation*}
    \begin{aligned}
      \frac{\partial^2 z(\bm{\alpha})}{\partial \alpha_i \partial \alpha_j}
      &= \frac{\partial M}{\partial \alpha_j} \bm{e}_{i}\bm{e}_{i}^\top(\bm{s} - P z(\bm{\alpha})) + M\bm{e}_{i}\bm{e}_{i}^\top \frac{\partial (\bm{s} - P z(\bm{\alpha}))}{\partial \alpha_j} \\
      &= -M\bm{e}_j\bm{e}_{j}^\top PM\bm{e}_{i}\bm{e}_{i}^\top (\bm{s} - P z(\bm{\alpha})) \\
&\quad + M\bm{e}_{i}\bm{e}_{i}^\top P(- M\bm{e}_{j}\bm{e}_{j}^\top (\bm{s} - P z(\bm{\alpha}))) \\
      &= (-M)(\bm{e}_j\bm{e}_{j}^\top PM\bm{e}_{i}\bm{e}_{i}^\top + \bm{e}_{i}\bm{e}_{i}^\top PM\bm{e}_{j}\bm{e}_{j}^\top )(\bm{s} - P z(\bm{\alpha}))
    \end{aligned}
  \end{equation*}

The Hessian matrix of $f( \alpha )$ is
\begin{align*}
\nabla^2 f(\bm{\alpha}) =
&-\textrm{Diag}(M\textbf{1})PM\textrm{Diag}(\bm{s} \\
&- P z(\bm{\alpha})) - (\textrm{Diag}(M\textbf{1})PM\textrm{Diag}(\bm{s} - P z(\bm{\alpha})))^\top
\end{align*}

For the matrix norm of this the following inequality holds.

\begin{equation*}
\begin{aligned}
\|\nabla^2 f(\bm{\alpha})\|_2 &\leq 2\|\textrm{Diag}(M\textbf{1})|\|_2\|P\|_2\|M\|_2\|\textrm{Diag}(\bm{s} - P z(\bm{\alpha}))\|_2
\end{aligned}
\end{equation*}

$M$ is bounded from Lemma~\ref{lm51}, so all terms of multiplication is bounded. This proves the theorem.

\end{proof}

\begin{lemma}\label{lem:lipschitz}
The gradient $\nabla f$ of the objective function $f$ is Lipschitz continuous over the feasible region.
\end{lemma}
\begin{proof}
$\|\nabla^2 f(\bm{\alpha})\|_2$ is bounded from Lemma~\ref{lem:boundedness}.
  By putting $L = \|\nabla^2 f(\bm{\alpha})\|_{2}^{2}$,
  mean-value theorem shows
  \begin{equation*}
    \bm{x}, \bm{y} \in \Omega,\ \|\nabla f(\bm{x}) - \nabla f(\bm{y})\| \leq L \| \bm{x} - \bm{y} \|
  \end{equation*}
\end{proof}


